Clapeyron.jl: An extensible, open-source fluid-thermodynamics toolkit

Thermodynamic models are often vital when characterising complex systems, particularly natural gas, electrolyte, polymer, pharmaceutical and biological systems. However, their implementations have historically been abstruse and cumbersome, and as such, the only options available were black-box commercial tools. In this article, we present Clapeyron.jl: a pioneering attempt at an open-source fluid-thermodynamics toolkit to build and make use of thermodynamic models. This toolkit is built in Julia, a modern language for scientific computing known for its ease of use, extensibility, and first-class support for differentiable programming. We currently support more models than any package available, including standard cubic (SRK, PR, PSRK, etc.), activity-coefficient (NRTL, UNIFAC, etc.), COSMO-based, and the venerable SAFT equations. The property-estimation methods supported are extensive, including bulk, VLE, LLE, VLLE and critical properties. With Clapeyron.jl, researchers and enthusiasts alike will be able to focus on the application and worry less about the implementation.

==> Makefile <==
TEXFLAGS = -e '$$pdflatex=q/pdflatex %O -shell-escape %S/' -pdf
LATEXMK = latexmk

PACKAGE = minted.dtx \
		  minted.ins \
		  minted.pdf \
		  README \
		  Makefile

.PHONY: minted all doc dist clean cleanall

minted: minted.sty

doc: minted.pdf

all: minted doc

minted.sty: minted.ins minted.dtx
	tex minted.ins

minted.pdf: minted.sty minted.gls minted.dtx
	$(LATEXMK) $(TEXFLAGS) minted.dtx

minted.gls: minted.glo
	makeindex -s gglo.ist -o minted.gls minted.glo

minted.glo: minted.dtx minted.sty
	$(LATEXMK) $(TEXFLAGS) minted.dtx

dist: $(PACKAGE)
	@$(RM) minted.zip
	@zip minted-$(shell grep '^\\ProvidesPackage' < minted.sty | grep -o '\<v[[:digit:]]*\.[[:digit:]]*\>').zip $(PACKAGE)

clean:
	@$(RM) *.aux *.log *.out *.toc *.fdb_latexmk *.ilg *.glo *.gls *.lol

cleanall: clean
	@$(RM) minted.sty minted.zip


==> content/why_julia.tex <==
\section{Why Julia?}
\label{sect:julia}
Julia is a high-performance programming language with relatively low barriers to entry, with a syntax that is as simple as Python, but with up to C-like performance with optimised code. It uses a just-in-time (JIT) compiler which means that code can be executed on an interactive terminal or on a notebook. Unlike Python, where most of the libraries are linked in the form of shared libraries from various compiled languages for performance (often referred to as the `two language' problem), in Julia, most of the libraries, including the ones in the Julia Standard Library, are written in pure Julia. This is indeed the case with \texttt{Clapeyron.jl}, in contrast to packages like \texttt{thermopack}, \texttt{feos} and \texttt{teqp} which are written in FORTRAN, Rust and C++, respectively, but all use Python front-ends. 

This means that \texttt{Clapeyron.jl} (and Julia packages in general) is highly transparent, and users are able to easily look into the implementation of every algorithm that they may be using and learn from or improve upon them where necessary. While there is a strong push from the community to keep everything in pure Julia whenever possible for that reason, it is also very easy to interface with existing libraries written in other languages (including Python).

\begin{figure}[bt]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/Clapeyron_structure.pdf}
    \caption{Architecture of the \texttt{Clapeyron.jl} package.}
    \label{fig:arch}
\end{figure}

Julia is specifically designed for scientific programming, and it boasts a syntax that allows for a near one-to-one translation of mathematical expressions, such as those in various thermodynamic models, to code without sacrificing efficiency. For example, the Carnahan-Starling equation for the reduced Helmholtz free energy of a hard-sphere, $a_\text{HS}$, is written mathematically as:
\begin{equation}
    a_\text{HS} = \frac{4\eta-3\eta^2}{(1-\eta)^2}\,,
\end{equation}
where $\eta$ is the packing fraction. In Julia, one can write:
\begin{minted}[breaklines,escapeinside=||,mathescape=true,  numbersep=1pt, gobble=2, frame=lines, fontsize=\small, framesep=2mm]{julia}
a_HS(η) = (4η-3η^2)/(1-η)^2
\end{minted}
The community strongly encourages making full use of the entire range of Unicode characters to better reflect how they are usually presented in the literature, where the use of the correct Greek characters and mathematical operators are common. It is also very easy to perform operations on arrays and matrices by broadcasting, which not only makes the code very clean, but also allows the compiler to optimise allocations at a low level.

Julia makes use of a multiple dispatch paradigm for code organisation, where functions are dynamically dispatched based on the types in the argument of the function call at run time. For example, we can define three separate functions:

\begin{minted}[breaklines,escapeinside=||,mathescape=true,  numbersep=1pt, gobble=2, frame=lines, fontsize=\small, framesep=2mm]{julia}
function f(x::Real)
    return x^2
end

function f(x::Float64)
    _x = floor(Int,x)
    return _x^2
end
\end{minted}
Here, we have three methods \texttt{f} defined for different input types. We can then see the effects of this multiple dispatch paradigm:

\begin{minted}[breaklines,escapeinside=||,mathescape=true,  numbersep=1pt, gobble=2, frame=lines, fontsize=\small, framesep=2mm]{julia}
julia> f(2)
4

julia> f(2.5)
4
\end{minted}
Based on the input, Julia will dispatch on the method with the input that has the closest type to the one used. We can see this above as, with \texttt{Float64} being a sub-type of \texttt{Real}, Julia used the second method in the case of the latter example above. 

Furthermore, whilst the example above focused on numeric types, developers in Julia can define their own types on which they can dispatch on. As a result, this allows programs that are written in Julia to be highly modular, such that any user is able to easily extend any functionality provided by third-party libraries without any modifications to the original source code, just by declaring the correct subtypes and dispatching on the correct function. \texttt{Clapeyron.jl} makes full use of this design feature to build a full-featured thermodynamics framework where users have complete control over every part of the software.

One interesting side-effect of Julia’s design is that it makes the implementation of automatic differentiation very natural. Users can, for example, write their own function of the Helmholtz free energy as a function of temperature, volume and the compositions, and any-order derivatives are immediately available for use in any of the thermodynamic methods provided by \texttt{Clapeyron.jl} without needing to be cognisant of what is happening behind the scenes. This is in stark contrast to how thermodynamic models are traditionally implemented, where every derivative has to be derived analytically (see \texttt{phasepy}\citep{Chaparro2020Phasepy:Computation} and \texttt{thermopack}\citep{Wilhelmsen2017ThermodynamicMethods}).
